End-to-End Rationale Reconstruction

The logic behind design decisions, called design rationale, is very valuable. In the past, researchers have tried to automatically extract and exploit this information, but prior techniques are only applicable to specific contexts and there is insufficient progress on an end-to-end rationale information extraction pipeline. Here we outline a path towards such a pipeline that leverages several Machine Learning (ML) and Natural Language Processing (NLP) techniques. Our proposed context-independent approach, called Kantara, produces a knowledge graph representation of decisions and of their rationales, which considers their historical evolution and traceability. We also propose validation mechanisms to ensure the correctness of the extracted information and the coherence of the development process. We conducted a preliminary evaluation of our proposed approach on a small example sourced from the Linux Kernel, which shows promising results.

==> text/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

%\bentley{The benefits/limitations/related work is good, but there's not enough space. The most important information should be placed into the intro, approach, or conclusion sections. For example, mention the subjective problem for rationale and the sentence-based extraction in the approach section.}







==> text/proposal_2.tex <==

\subsection{Response Generation.}

In response of a query, our proposed system should be able to present the user with a response. This is a two step process.
Our imagined scenario involves a person trying to understand the rationale behind a certain design decision. He formulates a query describing the design decision taken.

\todo{use the persona + example here to show better}
\todo{Bently: show better what's the impact of this part, give recommendations, what benefit is there to the user? how they would use the information?}
\todo{Bently suggestation: maybe a web inteeface, 
or github plugin ( a box that extracts + suggests) - add the autommaticlly suggestss part + recommednation part, 
}
\todo{Bently: a github bot for rationale as an application, start small , a simple bot that reads a KG format and give automatic messages/recommendations }

\begin{itemize}
    \item \textbf{Selection.} 
    In order to select relevant design decisions,  our proposed retrieval system comprises two main components 1) a decisions index and 2) a search algorithm to traverse the graph.
    The retrieval process has two steps: 
    \begin{enumerate}
        \item  Compute a relevance score (e.g. similarity score, or BM25 score ) to find and rank the relevant design decisions. In this step, we only consider an index of the design decisions nodes of our graph. We plan to experimentally propose a threshold and filter out  results with relevance scores
        below that threshold.
        
        \todo{ mention 8 and 13 in my IR survey  as related work that used LTR in Software design }
        
        \item  For each relevant design decision selected, we will leverage our decision-rationale graph to retrieve not only its corresponding rationale, but also the decisions K-edge away from the selected design decision, and their rationales. K will be determined experimentally but we predict that a value of 1 or 2 should be reasonable to justify a certain decision, and explain how it relates to other decisions.
        
        \todo{the 2 hop thing to give full recommendations?}
        
    \end{enumerate}
   
   Since design is contextual, it is important for the users to understand the context of the problem, that led the decision making. Thus we retrieve the context of the decision in order to make the utilization of the information less difficult.
   
 


 
   \todo{ Query based retrieval / SECTION 6.3 IN Design Rationale survey 2000  }
    
    \todo{-generic selection: citations 42 and 43 in OD3 paper}
    
    
    \todo{ 9.3. Retrieval - In Design Ratioanle survey 2000} 
    
    \todo{ https://www.sbert.net/docs/pretrained-models/msmarco-v2.html  }
    
     \todo{ look at KG/retreival workshop pointed out during IVADO workshops }
    
    
    
    
    
    %%%%%%%%%%%%%%%%
    \item \textbf{Synthesis and Presentation}.
    The user would be presented with a list of documents, each document corresponds to each design decision selected.
    Each document is composed a two parts: 1) an image of the sub-graph containing the decision selected, its rationale and its k-edges away decisions and their rationales. 2) a textual description of the image that  coherently integrates the sub graph information.
    
    
\todo{    Sarah Rastkar and Gail C Murphy. Why did this code change <-- leveraged more advanced summarization techniques with the use of multi-document extractive
summarization. They tried to generate concise natural language descriptions of the reasons resulting in a code change.
This information is useful to the developer as it allows him to make the right implementations choices and helps him
avoid collisions}


\todo {did they use synthesis ?? 
( generate a crowd cookbook of rationale and answer the question "why it is done?" using topic modeling ( like this paper where they answer 'how it is done?' ) % https://arxiv.org/pdf/1903.09174.pdf  
}
  
  
  -related work on synthesis (maybe template based) https://arxiv.org/pdf/2110.13283.pdf 
  
  
  \subsection{bot interactions ~ future work }
  The bot should be (besides retrieval):
  1 ) provide recommendations/suggestions (based on previous rationales, decisions..) that the user can accept/refuse 
  
  2) do an update mechanism when new decisions are added to make sure they are consistent + in addition to the quality checking the graph does after creating the graph for the first time.

related work on bots in SE : section 3.3 in \cite{saini2022automated}

\end{itemize}

%%%%%%% Benefits of retrieval part
*Given a design decision, finding
the relevant rationale information is a key pain point for engineers. The intensity of the problem multiplies in large organizations where different teams work on the same projects at different points in time. 

This decision-rationale graph would help in selecting relevant information to the user by taking into account how different decisions are interconnected.


To use a modelling bot
in learning environments, it is imperative that the queries can
be executed efficiently and their results can be obtained in realtime. Therefore, graph database management systems, e.g.,
Neo4j and platforms for question answering, e.g., AllenNLP
(see Figure 1) need to be explored.


%%%%%%%limitations of the retreival part
\textbf{Selection}: which \textbf{selection algorithm} to use (BM25, LTR, neural models?, we will do so feature engineering?, how we will do it in a generic way?, any graph based special Ir algorithms ? )  maybe use similarity on the embedding for retrieval selection ? % Automatically Matching Bug Reports With Related App Reviews . --> Deep Matcher, based on similarity of the embeddings,,  query-based selection for retreival    

textbf{Synthesis}

\textbf{Presentation}

although OD3 system needs personlization, for this project,we keep it for future improvement, 
    document request part (personalization, etc .... ) for future
+ selection based on the personlization for future also


-our retrieval is based on the decision and not on the rationale, our index is independent on the represenation of the rationale ....

%% retreival + usefulness challenges/limitations 
-\textbf{Relevance}, it is possible that the rationale captured at design time may not be relevant to those reviewing the rationale
at a later time in a different context \cite{horner2006effective}


